When Bousfield localizations and homotopy idempotent functors meet again

We adopt semimodel categories to extend fundamental results related to Bousfield localizations of model categories. More specifically, we generalize Bousfield-Friedlander Theorem and Hirschhorn Localization Theorem of cellular model categories to settings where their classical formulation does not apply. We use such results to answer, in the world of semimodel categories, an open problem posed by May-Ponto about the existence of Bousfield localizations for Hurewicz and mixed type model structures.

==> Contents/BousfieldFriedlanderCell.tex <==
In order to obtain right Bousfield localizations (or to study coreflective subcategories of homotopy categories), we may use the dual notion of that of localizator.

\begin{defn} Let $(\Mrect,\Eq)$ be a \textcolor{blue}{structured homotopical category} / relative category. A \emph{cellularizator} in $\Mrect$ is an augmented homotopical endofunctor $(\Qfrak\colon\Mrect\to\Mrect,\upepsilon\colon \Qfrak\Rightarrow\id)$ which induces a cellularization functor in $\Ho\M$. More precisely, $(\Qfrak,\upepsilon)$ satisfies:
	\begin{itemize}
		\item $\Qfrak$ preserves $\Eq$.
		\item $\Qfrak\upepsilon$ and $\upepsilon\Qfrak$ belong to (the saturation of) $\Eq$ (PUEDE RELAJARSE PERO NO SE SI PONERLO). 
	\end{itemize}
\end{defn}

\textcolor{blue}{CHECK:} Direction of cellularizators and steps.



%%%%%%%%%%%%% DEFINITION LEFT SEMIMODELS %%%%%%%%%%%%%%%%%%%

%\begin{defn} A \emph{left semimodel category} is a structured homotopical category $\M$ whose opposite structured homotopical category $\M^{\textup{op}}$ is a right semimodel.
%\end{defn}
%
%\begin{rem} More concretely, a Fresse left semimodel $\M$ satisfies:
%		\begin{itemize}
%		\item[(i)] (Lifting axioms) $\Cof_{\circ}\cap\Eq\boxslash\Fib$ and $\Cof_{\circ}\boxslash\Fib\cap\Eq$.
%		\item[(ii)] (Factorization axioms) Any map with cofibrant source can be factored either as $\Cof_{ \circ}\cap\Eq+\Fib$ or either as $\Cof_{\circ}+\Fib\cap\Eq$.
%		\item[(iii)] the initial object $\mathbb{0}$ is cofibrant.
%	\end{itemize}
%\end{rem}
%
%\begin{defn} Let $\M$ be a left semimodel category. A \emph{cellularizator} in $\M$ is an augmented homotopical endofunctor $(\Qfrak\colon\Mrect\to\Mrect,\upepsilon\colon \Qfrak\Rightarrow\id)$ which induces a cellularization functor in $\Ho\M$. More precisely, $(\Qfrak,\upepsilon)$ satisfies:
%	\begin{itemize}
%		\item $\Qfrak$ preserves $\Eq$.
%		\item $\Qfrak\upepsilon$ and $\upepsilon\Qfrak$ belong to (the saturation of) $\Eq$ (PUEDE RELAJARSE PERO NO SE SI PONERLO). 
%	\end{itemize}
%\end{defn}


With such device acting on a structured homotopical category $\M$, one may define distinguished classes of maps on the underlying category $\Mrect$.
\begin{defn}\label{defn_Cellularizator} Let $\Qfrak$ be a cellularizator in a \textcolor{blue}{structured homotopical category} / left semi-model $\M$. 
	\begin{itemize}
		\item An $\Qfrak$-equivalence is a map in $\Mrect$ whose image under $\Qfrak$ belongs to $\Eq$. The class of all $\Qfrak$-equivalences is denoted $\Eq_{\Qfrak}=\Qfrak^{-1}(\Eq)$.
		\item A $\Qfrak$-cofibration is a map with the llp with respect to all fibrations which are $\Qfrak$-equivalences. The class of $\Qfrak$-fibrations is denoted $\Cof_{\Qfrak}={}^{\boxslash}\big(\Fib\cap\Eq_{\Qfrak}\big)$.
		\item A $\Qfrak$-colocal object is an object $\Xrect\in\Mrect$ for which $\upepsilon_{\Xrect}\colon\Qfrak\Xrect\to\Xrect$ belongs to the saturation of $\Eq$.
	\end{itemize}
\end{defn}

Then, the dual result of Theorem \ref{thm_LBLfromLocalizator} stablishes that these classes always define a Fresse left semi-model structure if we start with one of them.
\begin{thm}\label{thm_RBLviaCellularizator} Let $\M=(\Mrect,\Cof,\Eq,\Fib)$ be a Fresse left semi-model and $\Qfrak$ a cellularizator in $\M$. Then, 
	$$
	\M_{\Qfrak}=(\Mrect,\Cof_{\Qfrak},\Eq_{\Qfrak},\Fib)
	$$
	is a Fresse left semimodel. In fact, $\M_{\Qfrak}$ is the right Bousfield localization of $\M$ at $\Qfrak$-equivalences. That is, it is initial between Fresse left semimodels $\OpN$ equipped with a right Quillen functor $\M\to\OpN$ which sends $\Eq_{\Qfrak}$ to equivalences.
\end{thm}



%%%%%%%%%%%%% EXAMPLE OF EXTENSION MODELSs %%%%%%%%%%%%%%%%%%%%%

%\begin{ex} Let $\upiota\colon \Op\to \OpP$ be a homotopical inclusion of admissible operads in $\V$. Then, the derived adjunction
%	$$
%	\mathbb{L}\upiota_{\sharp}\colon \Alg_{\Op}(\V)_{\text{proj}} \rightleftarrows \Alg_{\OpP}(\V)_{\text{proj}}\colon \upiota^*
%	$$
%	yields a cellularizator $\Qfrak=\mathbb{L}\upiota_{\sharp}\upiota^*$ over $\Alg_{\OpP}(\V)_{\text{proj}}$. The Fresse left semimodel $\Alg_{\OpP}(\V)_{\Qfrak}$ obtained from Theorem [\textcolor{red}{REF}] presents the homotopy theory of $\Op$-algebras inside $\OpP$-algebras.
%\end{ex}





%%%%%%%%%%%%%%%%%%% Relaxed variant %%%%%%%%%%%%%%%%%%%

%Additionally, the dual of Theorem [\textcolor{red}{REF}] also holds.
%\begin{thm}
%	Let $\M$ be a Fresse left $\Urect$-semimodel (i.e. $\M^{\textup{op}}$ is Fresse right \mbox{$\Urect^{\textup{op}}$-semimodel}) and $\Qfrak\colon\Mrect\to\Mrect$ a cellularizator which satisfies: for any pushout square in $\Mrect$
%	$$
%	\begin{tikzcd}[ampersand replacement=\&]
%	\Xrect \ar[rd, phantom, "\ulcorner"]\ar[d, "\upj"'] \ar[r, "\upg"] \& \Xrect'\ar[d]\; \\
%	\Yrect \ar[r, "\upg'"'] \& \Yrect',
%	\end{tikzcd}
%	$$
%	where $\Xrect'$ is $\Urect$-cofibrant and $\upj$ is a core $\Qfrak$-cofibration, the map $\upg'$ is an \mbox{$\Qfrak$-equivalence} provided $\upg$ is so. 
%	%that $\Rfrak$-equivalences between $\Urect$-fibrant objects are stable under pullbacks along $\Urect$-core fibrations. 
%	Then, 
%	$
%	\M_{\Rfrak}$
%	is a Fresse left $\Urect$-semimodel.
%\end{thm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%% COMMENTS ON HOW ONE CANNOT LIFT THE THEOREM TO SPITZWECK SEMIMODELS %%%%%%%%%%%%%%%%%%%



%\begin{rem}
%	There is a more common variant of semimodel structure which first appeared in Hovey's work on model categories on monoids [\textcolor{red}{REF}] and which was more throughly explored in Spitzweck's thesis [\textcolor{red}{REF}]. They are Fresse right (resp. left) semimodels such that $(\Cof\cap\Eq,\Fib)$ (resp. $(\Cof,\Fib\cap\Eq)$) is a full weak factorization system [\textcolor{red}{REF}]. Following  [\textcolor{red}{REF}], we call them \emph{Spitzweck semimodel structures}. 
%
%    The main Theorems [\textcolor{red}{REF}] are not automatically true for Spitzweck semimodels, but all the obstruction is the apparent lack of the remainig factorization for all morphisms. As observed in the original Bousfield-Friedlander theorem, one may ask a stability condition on $\Rfrak$-equivalences (similar to the one of Theorems [\textcolor{red}{REF}]) in order to have this last factorization, but then, working with Spitzweck semimodels in place of full model structures does not bring any advantages.
%\end{rem}





==> Contents/Intro.tex <==
\paragraph{Motivation and main results.} Idempotent functors are an effective tool to coherently discard information and, as a fundamental idea, they are widespread across mathematics: from group theory and topology to algebraic geometry and logic among many other areas. A particularly interesting example related to all the previous areas is given by sheafification. Given a Grothendieck topology, sheafification is an idempotent functor which forgets all the information that is not local with respect to that topology. In categorical terms, such idempotent functors are (co)reflectors into full subcategories, i.e.\;left (resp.\;right) adjoint functors for inclusions of full subcategories.

If one is willing to consider also a homotopical context in the recipe, which we simply denote by $\M\to\Ho\M$, one arrives at the notion of homotopy idempotent functor, i.e. idempotent functors for $\Ho\M$ which live at the point set level $\M$. To be more precise, let $\M$ be a model category. A coaugmented homotopy idempotent functor\footnote{For the sake of conciseness, we refer to them as BF-reflectors in the body of the paper.} is a functorial construction $\Lrect$ on $\M$ which preserves equivalences and which is equipped with a natural comparison map $\id\Rightarrow \Lrect$ that becomes an equivalence when combined with $\Lrect$ in the two obvious ways to produce $\Lrect\Rightarrow\Lrect^2$. As expected, such $\Lrect$ on $\M$ produces a reflexive subcategory of $\Ho\M$, the full subcategory spanned by $\Lrect$-local objects. An object $\Xrect$ is $\Lrect$-local if the comparison map $\Xrect\to\Lrect\Xrect$ is an equivalence. Such objects are those that do not contain forgettable information with respect to $\Lrect$. Maps that $\Lrect$ sees as equivalences, called $\Lrect$-equivalences, are those maps that measure when two objects are indistinguishable when using $\Lrect$ to forget the selected information.

Why is this new intricacy introduced if we just want idempotent functors on $\Ho\M$? %The answer comes from the dawn of such functorial ways to forget information.
The frequent lack of good properties of homotopy categories, such as existence of (co)limits, usually hinders the task of constructing idempotent functors on $\Ho\M$. Working on $\M$ allows one to use homotopical constructions instead. 
 %For instance, the Quillen model structure presenting the homotopy theory of spaces, $\mathsf{sSet}_{\Qrect}\to\Ho\Spc$, was particularly useful in the landmark work of Bousfield and its.

One of many of Bousfield's bright ideas was to interprete homotopy idempotent functors as fibrant or cofibrant replacements in a new model category constructed from $\M$: enlarge the class of equivalences, %considering $\Lrect$-equivalences, 
fix the class of cofibrations or fibrations and check if the resulting structure is a model category. % Bousfield localizations are named %after a direction corresponding to the direction of the natural comparison map that comes with the homotopy idempotent functor, i.e. left or right means $\id\Rightarrow\Lrect$ or $\Lrect\Rightarrow\id$ respectively.
%left or right if the comparison is $\id\Rightarrow\Lrect$ or $\Lrect\Rightarrow \id$ respectively\footnote{In the literature, right Bousfield localizations are also called cellularizations.}. 
Thus, homotopy idempotent functors can be found through the production of Bousfield localizations of model categories.  

This work reverses this approach, i.e.\;we show that Bousfield localizations exist as long as homotopy idempotent functors are present. Hence, one can apply model categorical techniques to study (co)reflexive subcategories of $\Ho\M$ in great generality.

The fundamental idea was already present in \cite{bousfield_homotopy_1978}, where Bousfield and Friedlander give a famous method to construct Bousfield localizations from particularly nice homotopy idempotent functors and nice model categories. Our contribution in this respect is that working with semimodel categories instead of full model categories enables one to always construct the associated Bousfield localization\footnote{There are subtleties concerning the notion of semimodel category that one has to use.}.
\begin{taggedtheorem}{\textbf{A}}[Theorem \ref{thm_LBLfromLocalizator}] \label{thm_A_LocalizatorLBL}
Let $\M$ be a (right semi)model category and $\id\Rightarrow\Lrect$ a coaugmented homotopy idempotent functor. Then, $\M$ admits a left Bousfield localization at $\Lrect$-equivalences among right semimodel categories.
\end{taggedtheorem}

%Semimodel structures are a generalization of model categories for which lifting and factorization axioms are relaxed by restricting (co)domains of the maps involved. 

It is important to note that right semimodel structures appear naturally when constructing left Bousfield localizations through this theorem. This fact has to be compared with different existence theorems for left Bousfield localizations that have appeared in the literature (see \emph{Relation to other works} below) that assert existence of left Bousfield localizations among left semimodel categories. These results correspond to the construction of left Bousfield localizations at classes of equivalences generated by sets of maps. In fact, we also provide an instance of them which may be well-known to experts. It concerns (enriched) left Bousfield localization of cellular model structures at a set of maps and covers what happens in the absence of left properness in \cite[Theorem 4.1.1]{hirschhorn_model_2003}.

\begin{taggedtheorem}{\textbf{B}}[Theorem \ref{thm_BousfieldLocalizationCellularCase}]\label{thm_B_CellularLBL} Let $\M$ be a cellular (left semi)model category whose generating sets have cofibrant domains and $\Srect$ a set of maps in $\M$. Then, the left Bousfield localization of $\M$ at $\Srect$ exists among left semimodel categories.
\end{taggedtheorem}  

The difference between both theorems can be explained as follows. Recall that a model category $\M$ has two interacting weak factorization systems. When constructing a left Bousfield localization, one tries to modify the one corresponding to acyclic cofibrations and fibrations to accomodate the new fibrant objects or the new equivalences. Depending on which side one is willing to relax, the difference appears: the factorization and the lifting axioms for the new classes (acyclic cofibrations, fibrations) are restricted to maps with nice domains (left semimodel) or to maps with nice codomains (right semimodel).

On the one hand, Theorem \ref{thm_B_CellularLBL} may be seen as the companion of \cite[Theorem A]{white_left_2020}, where left Bousfield localization of (tractable) combinatorial model categories is discussed. Its principal applications are given by studying left Bousfield localizations of non left-proper model categories constructed from topological spaces equipped with the Quillen model structure.

On the other hand, Theorem \ref{thm_A_LocalizatorLBL} and its dual are more flexible in many respects. To justify this claim, we discuss (enriched) left Bousfield localization at a set of maps assuming neither cellularity nor combinatoriality.

\begin{taggedtheorem}{\textbf{C}}[Theorem \ref{thm_LBLatSequivalencesWith1StepLocalizator}]\label{thm_C_LBLatSetOfMaps}
Let $\M$ be a left proper (right semi)model category and $\Srect$ a set of maps in it. If (i) $\M$ has a set of maps $\Jrect$ such that fibrant objects in $\M$ are those that admit liftings against $\Jrect$, and (ii) a  certain set of maps admits Quillen's small object argument\footnote{Or any generalization which produces factorizations whose left factor is a cellular complex.}, the left Bousfield localization of $\M$ at $\Srect$ exists among right semimodel categories.  
\end{taggedtheorem}

We exploit the simple ideas behind Theorem \ref{thm_C_LBLatSetOfMaps} to answer, in the realm of semimodel categories, an open question of May and Ponto in \cite{may_more_2012}. By Hirschhorn's theory of localizations of cellular model categories \cite{hirschhorn_model_2003}, the Quillen model structure on topological spaces is known to admit the left Bousfield localization at any set of maps. However, there are two non cellular model structures on topological spaces which are not known to admit such localizations; these are the Hurewicz and the mixed model structure (see \cite[Remark 19.5.7]{may_more_2012}). 

\begin{taggedtheorem}{\textbf{D}}[Propositions \ref{prop_LocalizationsOfHurewiczMixedModelsSIMPLICIALCASE} and \ref{prop_LocalizationsOfHurewiczMixedModelsTOPOLOGICALCASE}]
The Hurewicz and the mixed model structure on the category of topological spaces admit left Bousfield localizations at any set of maps among right semimodel categories.
\end{taggedtheorem} 

In fact, we distinguish between two ways to localize these model structures at a set of maps, we discuss right Bousfield localizations and our methods also apply to Hurewicz and mixed model structures on chain complexes (see Section \ref{sect_Applications}).

To conclude this motivation, we note that the dual of Theorem \ref{thm_A_LocalizatorLBL} has been applied to construct new model structures in the settings of algebraic quantum field theories and factorization algebras in \cite{carmona_algebraic_2021, carmona_model_2021}. See Section \ref{sect_Applications} for more on this.


\paragraph{Relation to other works.} For nice introductions to (homotopy) idempotent functors and Bousfield localizations, together with a plethora of examples where such techniques can be applied, see  \cite{dwyer_localizations_2004,lawson_introduction_2020}. 

Theorem \ref{thm_A_LocalizatorLBL} is just a convenient variation of Bousfield-Friedlander's Theorem, which originally appeared in \cite{bousfield_homotopy_1978}. Enhancements of this result are given in \cite{biedermann_duality_2015, bousfield_telescopic_2001, stanculescu_note_2008}. In particular, Proposition \ref{prop_LBLForNonFunctorialBFReflectors} generalizes Theorem \ref{thm_A_LocalizatorLBL} to incorporate Biedermann-Chorny's idea \cite[Appendix A]{biedermann_duality_2015}.

Regarding left and right Bousfield localizations of cellular model categories, the principal reference is Hirschhorn's book \cite{hirschhorn_model_2003}. In fact, our exposition and results owes a lot to this work. Hirschhorn's general localization results, together with Smith's Theorem \cite[Proposition 2.2]{barwick_left_2010}, are the most applied techniques in the literature concerning Bousfield localizations. However, both approaches require properness asumptions to work. Fortunately, several people 
 observed that Bousfield localizations exist in some cases as semimodel categories without assuming properness asumptions and they deduced important results from this fact.    

When lacking left properness, the existence of left Bousfield localization for combinatorial (left semi)model categories is addressed in \cite{henry_combinatorial_2020,white_left_2020}. Indeed, Batanin-White \cite[Theorem B]{white_left_2020} generalize Smith's Theorem to combinatorial left semimodel categories and they  provide a thorough list of possible applications. Regarding non left proper cellular model categories, Goerss-Hopkins \cite{goerss_moduli_2005} and Harper-Zhang \cite{harper_topological_2019} showed that certain homological localizations of operadic algebras exist. However, to the best of our knowledge, no general result appearing in the literature provides a parallel to the standard reference \cite{hirschhorn_model_2003} about existence of left Bousfield localization for cellular model categories. Theorem \ref{thm_B_CellularLBL} fills this gap. 

\paragraph{Outline.} Section \ref{sect_Preliminaries} contains basic definitions of semimodel categories and an original discussion of Quillen functors and bifunctors between them. This is needed in order to compare left and right semimodel categories (Proposition \ref{prop_WeakQuillenPairsInduceAdjunctions} and Remark \ref{rem_CoreAdjunctions}) and to have a sound theory of enrichment for semimodel categories (Proposition \ref{prop_CoreQuillenAdjOfTwoVariablesYieldAdjunctionsOfTwoVariables} and Remark \ref{rem_EnrichmentOfSemimodels}). Theorem \ref{thm_A_LocalizatorLBL} and its proof constitutes Section \ref{sect_LBLviaLocalizators}. The bridge between Theorems \ref{thm_A_LocalizatorLBL} and \ref{thm_B_CellularLBL} is constructed in Section \ref{sect_LocalizatorsFromSmallData}, where we try to obtain a coaugmented homotopy idempotent functor which corresponds to left Bousfield localization at a set of maps. The cited section contains Theorem \ref{thm_C_LBLatSetOfMaps}. Left Bousfield localization of non left-proper cellular model categories is addressed in Section \ref{sect_LBLviaCellularity} and it leads up to Theorem \ref{thm_B_CellularLBL}. Finally, Section \ref{sect_Applications} is comprised of examples and applications of the main results.


\paragraph{Conventions:} We will freely use reduced notations for basic notions in the theory of model categories. For instance, \emph{llp} (resp. \emph{rlp}) refers to left (resp. right) lifting property, $\upi\boxslash\upp$ means $\upi$ satisfies llp with respect to $\upp$, \emph{wfs} means weak factorization system, \emph{soa} denotes small object argument, etc.

==> Contents/PackagesAndOperators.tex <==
\usepackage[english,activeacute]{babel}
\usepackage{etex}
\usepackage[latin1]{inputenc}
\usepackage[all]{xy}
\usepackage[latin1]{inputenc}
\usepackage{xypic,color}
\usepackage{latexsym}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{wasysym}
\usepackage{mathrsfs}
\usepackage{euscript}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{cancel}
\usepackage{graphicx,color}
\usepackage{multicol}
\usepackage{color}
\usepackage{multirow}
\usepackage{makeidx}
\usepackage{upgreek}
\usepackage{setspace} 
\usepackage{import}
\usepackage{float}
\usepackage{mleftright}
\usepackage{stmaryrd}
\usepackage{diagbox}

%BINOMIOS CON BRACKETS PARA MAPPING SPACES
\newcommand{\brbinom}[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}

%\usepackage{scalerel}
%%\setlength{\oddsidemargin}{0mm} 
%%\setlength{\hoffset}{0mm}
%\setlength{\textwidth}{200mm}
%\setlength{\oddsidemargin}{-3mm}
%\setlength{\evensidemargin}{-3mm} 
%\setlength{\textheight}{240mm}   %Estaba en 245
%%\setlength{\topmargin}{-8mm}





\usepackage{bbold}

%\usepackage[all, 2cell]{xy}
%\UseAllTwocells


\usepackage{tikz}
\usepackage{tikz-cd}
\usetikzlibrary{matrix,arrows,calc,decorations.pathmorphing,fit,shapes.geometric,decorations.pathreplacing,positioning,snakes}

%\usepackage{tikz}

\usepackage{xcolor}
\definecolor{babyblueeyes}{rgb}{0.54, 0.81, 0.94}
\definecolor{blizzardblue}{rgb}{0.67, 0.9, 0.93}
\definecolor{blue(munsell)}{rgb}{0.0, 0.5, 0.69}
\definecolor{bluegray}{rgb}{0.4, 0.6, 0.8}
\definecolor{bondiblue}{rgb}{0.0, 0.58, 0.71}
\definecolor{cadetblue}{rgb}{0.37, 0.62, 0.63}
\definecolor{carolinablue}{rgb}{0.6, 0.73, 0.89}
\definecolor{cinnamon}{rgb}{0.82, 0.41, 0.12}
\definecolor{darkcandyapplered}{rgb}{0.64, 0.0, 0.0}
\definecolor{darkcyan}{rgb}{0.0, 0.55, 0.55}
\definecolor{darkmidnightblue}{rgb}{0.0, 0.2, 0.4}
\definecolor{darkpastelblue}{rgb}{0.47, 0.62, 0.8}
\definecolor{frenchblue}{rgb}{0.0, 0.45, 0.73}

%\newcommand{\contrastcolor}{frenchblue}%{Blue3}
%\newcommand{\headingscolor}{frenchblue}
\usepackage{url}
\usepackage[bookmarksopen,colorlinks,allcolors=frenchblue,urlcolor=frenchblue]{hyperref}



\makeindex

\usepackage{scalerel}

%\usepackage[applemac]{inputenc}  % Para TeXShop

%\setlength{\oddsidemargin}{0mm} 
%\setlength{\hoffset}{0mm}
%\setlength{\textwidth}{165mm}
%\setlength{\oddsidemargin}{-2.5mm}
%\setlength{\evensidemargin}{-2.5mm} 
%\setlength{\textheight}{245mm}
%\setlength{\topmargin}{-8mm}

%\usepackage{hyperref}
\usepackage{wrapfig}
\usepackage{ifpdf}

\usepackage{syntonly}
%\includeonly{Doc_b}

\DeclareMathOperator{\ob}{\mathsf{ob}}
\DeclareMathOperator{\id}{\mathsf{id}}

\DeclareMathOperator{\hocolim}{\mathsf{hocolim}}
\DeclareMathOperator{\holim}{\mathsf{holim}}
\DeclareMathOperator{\col}{\mathsf{col}}
\DeclareMathOperator{\source}{\mathsf{s}}
\DeclareMathOperator{\target}{\mathsf{t}}

\DeclareMathOperator{\upa}{\textup{a}}
\DeclareMathOperator{\upk}{\textup{k}}
\DeclareMathOperator{\upe}{\textup{e}}
\DeclareMathOperator{\upf}{\textit{f}}
\DeclareMathOperator{\upg}{\textit{g}}
\DeclareMathOperator{\uph}{\textit{h}}
\DeclareMathOperator{\upi}{\textit{i}}
\DeclareMathOperator{\upj}{\textit{j}}
\DeclareMathOperator{\upn}{\textup{n}}
\DeclareMathOperator{\upm}{\textup{m}}
\DeclareMathOperator{\upr}{\textup{r}}
\DeclareMathOperator{\upb}{\textup{b}}
\DeclareMathOperator{\upo}{\textup{o}}
\DeclareMathOperator{\upp}{\textit{p}}
\DeclareMathOperator{\upq}{\textit{q}}
\DeclareMathOperator{\upt}{\textup{t}}
\DeclareMathOperator{\upu}{\textit{u}}
\DeclareMathOperator{\upc}{\textup{c}}
\DeclareMathOperator{\upd}{\textup{d}}
\DeclareMathOperator{\upv}{\textit{v}}

\DeclareMathOperator{\C}{\EuScript{C}}
\DeclareMathOperator{\Op}{\EuScript{O}}
\DeclareMathOperator{\E}{\EuScript{E}}
\DeclareMathOperator{\D}{\EuScript{D}}

\DeclareMathOperator{\M}{\EuScript{M}}
\DeclareMathOperator{\OpN}{\EuScript{N}}
\DeclareMathOperator{\OpB}{\EuScript{B}}
\DeclareMathOperator{\OpI}{\EuScript{I}}
\DeclareMathOperator{\OpQ}{\EuScript{Q}}
\DeclareMathOperator{\OpP}{\EuScript{P}}


\DeclareMathOperator{\V}{\EuScript{V}}
\DeclareMathOperator{\Scurl}{\EuScript{S}}

\DeclareMathOperator{\Frect}{\mathsf{F}}
\DeclareMathOperator{\Srect}{\mathsf{S}}
\DeclareMathOperator{\Grect}{\mathsf{G}}
\DeclareMathOperator{\Xrect}{\mathsf{X}}
\DeclareMathOperator{\Yrect}{\mathsf{Y}}
\DeclareMathOperator{\Zrect}{\mathsf{Z}}
\DeclareMathOperator{\Trect}{\mathsf{T}}
\DeclareMathOperator{\Nrect}{\mathsf{N}}
\DeclareMathOperator{\Mrect}{\mathsf{M}}
\DeclareMathOperator{\Qrect}{\mathsf{Q}}
\DeclareMathOperator{\Rrect}{\mathsf{R}}
\DeclareMathOperator{\Arect}{\mathsf{A}}
\DeclareMathOperator{\Brect}{\mathsf{B}}
\DeclareMathOperator{\Crect}{\mathsf{C}}
\DeclareMathOperator{\Vrect}{\mathsf{V}}
\DeclareMathOperator{\Wrect}{\mathsf{W}}
\DeclareMathOperator{\Urect}{\mathsf{U}}
\DeclareMathOperator{\Drect}{\mathsf{D}}
\DeclareMathOperator{\Orect}{\mathsf{O}}
\DeclareMathOperator{\Irect}{\mathsf{I}}
\DeclareMathOperator{\Jrect}{\mathsf{J}}
\DeclareMathOperator{\Lrect}{\mathsf{L}}
\DeclareMathOperator{\Krect}{\mathsf{K}}
\DeclareMathOperator{\Erect}{\mathsf{E}}


\DeclareMathOperator{\ACof}{\mathsf{ACof}}
\DeclareMathOperator{\AFib}{\mathsf{AFib}}
\DeclareMathOperator{\Cof}{\mathsf{Cof}}
\DeclareMathOperator{\Fib}{\mathsf{Fib}}



\DeclareMathOperator{\Rfrak}{\mathfrak{R}}
\DeclareMathOperator{\Qfrak}{\mathfrak{Q}}
\DeclareMathOperator{\Dfrak}{\mathfrak{D}}

\DeclareMathOperator{\Ho}{\mathsf{Ho}}
\DeclareMathOperator{\Fun}{\mathsf{Fun}}
\DeclareMathOperator{\Eq}{\mathsf{Eq}}
\DeclareMathOperator{\Map}{\mathsf{Map}}
\DeclareMathOperator{\HOM}{\EuScript{H}\mathsf{om}}
\DeclareMathOperator{\h}{\mathsf{h}}
\DeclareMathOperator{\Mult}{\mathsf{Mult}}
\DeclareMathOperator{\Loc}{L}


\DeclareMathOperator{\chupachup}{\scaleobj{0.6}{\multimap}}
\DeclareMathOperator{\chupachups}{\rotatebox{90}{$\chupachup$}}



\DeclareMathOperator{\Ch}{\mathsf{Ch}}

\DeclareMathOperator{\emp}{{\raisebox{.4mm}{\o}}}
\DeclareMathOperator{\pt}{\mathrm{pt}}
%\DeclareMathOperator{\lim}{lim}

\DeclareMathOperator{\colim}{colim}
\DeclareMathOperator{\Spc}{\EuScript{S}pc}
\DeclareMathOperator{\Spt}{\EuScript{S}pt}
\DeclareMathOperator{\Alg}{\mathsf{Alg}}
\DeclareMathOperator{\pFac}{\mathsf{pFac}}
\DeclareMathOperator{\Fac}{\mathsf{Fac}}

\DeclareMathOperator*{\Bigcdot}{\scalerel*{\cdot}{\bigodot}}

\newcommand{\inters}[1]{\underset{#1}{\wedge}}


\usepackage{titlesec}

%\titleformat{\chapter}[hang]
%{\vspace{-3cm}
%\normalfont\LARGE\bfseries
%}{
%\chaptertitlename\:\, 
%\thechapter}{14pt}{}
%\titleformat{\section}[hang]
%{\vspace{0pt}
%\normalfont\Large\bfseries
%}{
%\chaptertitlename\:\, 
%\thesection}{14pt}{}
%\titleformat{\subsection}[hang]
%{\vspace{0pt}
%\normalfont\large\bfseries
%}{
%\chaptertitlename\:\, 
%\thesubsection}{14pt}{}


%\titleformat{\chapter}[hang]{\scshape}{}{0pt}
%\titleformat{\section}[block]{\scshape}{}{0pt}%{hbefore-codei}[hafter-codei]



\usepackage{float}

\usepackage{fancyhdr}
\pagestyle{fancy}
%\renewcommand{\chaptermark}[1]{\markboth{#1}{}} 
%\renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}}\fancyfoot[C]{\slshape \thepage}
% encabezados
%\lhead[\textcolor{frenchblue}{\thepage}]{\rightmark}
%\chead[]{}
%\rhead[\leftmark]{\textcolor{frenchblue}{\thepage}}
%\renewcommand{\headrulewidth}{0.5pt}

%\fancyhf{}
%\fancyhead[RE]{\nouppercase{\slshape\leftmark}}
%\fancyhead[LO]{\nouppercase{\slshape\rightmark}}
%\fancyhead[LE,RO]{\bfseries\thepage}


% pie y alto de pagina
\lhead[]{}
\chead[]{}
\rhead[]{}
\renewcommand{\headrulewidth}{0pt}
%\lfoot[]{}
%\cfoot[]{}
%\rfoot[]{}
%\renewcommand{\footrulewidth}{0pt}

% primera pagina de un capitulo
%\fancypagestyle{plain}{
%	\fancyhead[L]{}
%	\fancyhead[C]{}
%	\fancyhead[R]{}
%	\fancyfoot[L]{}
%	\fancyfoot[C]{}
%	\fancyfoot[R]{}
%	\renewcommand{\headrulewidth}{0pt}
%	\renewcommand{\footrulewidth}{0pt}
%}





\renewcommand{\thefootnote}{\roman{footnote}}



%FLECHA DE FUNCTOR GENERALIZADA


\usepackage{tikz}
\usetikzlibrary{calc,decorations.pathmorphing,shapes}

\newcounter{sarrow}
\newcommand\xrsquigarrow[1]{%
\stepcounter{sarrow}%
\mathrel{\begin{tikzpicture}[baseline= {( $ (current bounding box.south) + (0,-0.5ex) $ )}]
\node[inner sep=.5ex] (\thesarrow) {$\scriptstyle #1$};
\path[draw,<-,decorate,
  decoration={zigzag,amplitude=0.7pt,segment length=1.2mm,pre=lineto,pre length=4pt}] 
    (\thesarrow.south east) -- (\thesarrow.south west);
\end{tikzpicture}}%
}


==> Contents/ReflexiveSubcategoriesOfHomotopyCats.tex <==
As a brief aside, we show that Proposition \ref{prop_LocalizatorFromAlmostNothing} already produces a reflexive subcategory without assuming that $\M$ is left proper. In fact, we prove a result which is much more general than this observation but quite elementary from an appropiate point of view. 

What we prove only requires working on a relative category $(\Mrect,\Eq)$. Therefore, in the rest of this section, we consider a relative category $\M=(\Mrect,\Eq)$. For simplicity, we assume that $\Eq$ is saturated as a subcategory of equivalences. 
 
Localizing $\Mrect$ at $\Eq$ produces an $\infty$-category $\underline{\Ho}\M$ (with an appropiate universal property, see \cite[Section 7.1]{cisinski_higher_2019}) which enhances the ordinary localization $\Ho\M$\footnote{We will not deal with the usual set theoretic issues to construct localizations in general, we just assume that $\underline{\Ho}\M$ exists.}. Hence, we obtain three levels in which we can work: point set level ($\Mrect$), homotopy coherent level ($\underline{\Ho}\M$) and plain homotopy level ($\Ho\M$).

Our goal is to show that the following generalization of BF-reflector  (Definition \ref{defn_BFReflector}) produces a reflexive subcategory of $\underline{\Ho}\M$, and obviously of $\Ho\M$.     

\begin{defn} Let $\M$ be a relative category. A \emph{h-reflector} in $\M$ is an endofunctor $\Rfrak\colon\Mrect\to\Mrect$ equipped with a zigzag of natural transformations
	$$
	\upeta\colon \id\Leftarrow\cdots\Rightarrow\bullet\Leftarrow\cdots\Rightarrow\Rfrak
	$$
	whose left pointing components are all natural equivalences and which satisfies: 
	\begin{itemize}
		\item[($i$)] $\Rfrak$ is homotopical (as all the intermediate functors in the zigzag).
		\item[($ii$)] $\Rfrak\upeta$ and $\upeta\Rfrak$ are zigzags of natural equivalences. 
	\end{itemize}
	
	We will denote by $\upeta\colon \id\rightsquigarrow\Rfrak$ zigzags of natural transformations as above.
\end{defn}

\begin{defn} Let $\Rfrak$ be a h-reflector in a relative category $(\Mrect,\Eq)$. 
	\begin{itemize}
		\item An $\Rfrak$-equivalence is a map $\upf$ in $\Mrect$ such that $\Rfrak(\upf)$ is an equivalence. The class of all $\Rfrak$-equivalences is denoted $\Eq_{\Rfrak}=\Rfrak^{-1}(\Eq)$.
		
		\item A $\Rfrak$-local object is an object $\Xrect\in\Mrect$ for which $\upeta_{\Xrect}\colon\Xrect\rightsquigarrow\Rfrak\Xrect$ consists of equivalences. 
	\end{itemize}
\end{defn}

\begin{prop}\label{prop_LocalizatorInGeneralYieldsReflector} Let $\M$ be a relative category and $(\Rfrak,\upeta)$ a h-reflector in $\M$. Then, $\Rfrak$ induces a reflector of $\underline{\Ho}\M$ into its full subcategory of $\Rfrak$-local objects. In fact, $\Rfrak$ identifies the localization of $\underline{\Ho}\M$ at $\Eq_{\Rfrak}$ with such reflexive subcategory. The analogous statement holds replacing $\underline{\Ho}\M$ by $\Ho\M$.
	
In particular, the full subcategory of $\Rfrak$-local objects admits all homotopy (co)limits that $\underline{\Ho}\M$ has and they can be computed  using $\Rfrak$ and those of $\underline{\Ho}\M$.
\end{prop}
\begin{proof}
	Let us denote by $\underline{\mathsf{ho}}(\Rfrak\text{-local})$ the subcategories mentioned in the statement. Since $\Rfrak$ is homotopical, by the universal property of the localization and the definition of $\Rfrak$-local object, we obtain a functor
	$$
	\Rfrak\colon \underline{\Ho}\M\longrightarrow \underline{\mathsf{ho}}(\Rfrak\text{-local}).
	$$
	Similar reasons applied to $\upeta\colon\id\rightsquigarrow\Rfrak$ yield an homonomous zigzag of natural transformations $\upeta$ between endofunctors of $\underline{\Ho}\M$. Choosing inverses to the left pointing arrows in $\upeta$ and choosing a composition for the resulting chain of composable maps (both choices are essentially unique in the $\infty$-categorical sense), we get a natural transformation $\widetilde{\upeta}\colon\id\Rightarrow\Rfrak$ in $\underline{\Ho}\M$ such that $\Rfrak\widetilde{\upeta}$ and $\widetilde{\upeta}\Rfrak$ are equivalences. This data suffices to prove that $\Rfrak$ is left adjoint to the inclusion functor $\upi\colon \underline{\mathsf{ho}}(\Rfrak\text{-local}) \hookrightarrow\underline{\Ho}\M$ by \cite[Lemma 2.1.11 and Proposition 4.1.1]{riehl_elements_2022}. 
	
	 The equivalence between $\underline{\mathsf{ho}}(\Rfrak\text{-local})$ and the localization of $\underline{\Ho}\M$ at $\Eq_{\Rfrak}$ can be shown by checking that $\Rfrak\colon \underline{\Ho}\M\to\underline{\mathsf{ho}}(\Rfrak\text{-local})$ satisfies the appropiate universal property, which follows from (i) $\Rfrak$-equivalences between $\Rfrak$-local objects are equivalences and (ii) for any $\Xrect\in\M$, the zigzag $\upeta_{\Xrect}$ consists of $\Rfrak$-equivalences. 
\end{proof}

\begin{rem} The full subcategory of $\underline{\Ho}\M$ (resp. $\Ho\M$) spanned on $\Rfrak$-local objects may not coincide with the localization at $\Eq$ of the full subcategory of $\Rfrak$-local objects in $\Mrect$. However, they coincide if, for instance, $\M$ admits a homotopy 3-arrow calculus \cite{thomas_3-arrow_2011} or if $\M$ can be equipped with a semimodel structure.
\end{rem}

\begin{cor} Let $\M$ be a $\V$-(semi)model category and $\Srect$ a set of maps in it. Assume that (i) $\V$ admits a set of generating cofibrations with cofibrant sources, (ii) $\M$ admits a set of core acyclic cofibrations that detect fibrant objects and (iii) the set of maps   $\overline{\mathsf{Horn}}(\Srect)$ admits Quillen's soa. Then, $\underline{\Ho}(\Srect\textup{-local})$ is a reflexive subcategory of $\underline{\Ho}\M$.
\end{cor}


==> Contents/SOAsAndCells.tex <==
We briefly recollect some \emph{small object arguments} that have been proposed in the literature. Our aim is to write down a list of conditions under which small object arguments apply with an eye towards applications. 

\paragraph{Small Object Arguments.} 
By small object argument (soa), we understand a procedure that takes a ``small amount of data" in a category $\Mrect$ and gives back a weak factorization system $(\Lrect,\Rrect)$. The cornerstone is usually showing that the factorization axiom holds, i.e. given a map $\upf$, find a factorization
$$
	\upf\colon\bullet\xrightarrow{\quad{}\Lrect\quad}\bullet\xrightarrow{\quad\Rrect\quad}\bullet.
$$ 
This is usually achieved by a transfinite construction that iteratively adds solutions for all right lifting problems specified by the small amount of data. Thus, an essential ingredient in such procedures is to provide conditions under which this transfinite construction stops and yields the desired factorization. We strongly recommend \cite{riehl_categorical_2014} to more on weak factorization systems and small object arguments.

The most common soa is due to Quillen. One can find the precise constrution in \cite{hirschhorn_model_2003,hovey_model_1999,may_more_2012}. It takes a set of maps $\EuScript{K}$ as input and produces the weak factorization system $({}^{\boxslash}(\EuScript{K}^{\boxslash}),\EuScript{K}^{\boxslash})$. The factorization for a map $\upf$ using Quillen's soa produces
$$
\upf\colon \bullet\xrightarrow{\quad \EuScript{K}\text{-cell}\quad}\bullet\xrightarrow{\quad\EuScript{K}^{\boxslash}\quad}\bullet
$$
and it works whenever the domains of elements in $\EuScript{K}$ are small relative to $\EuScript{K}$. Recall that $\EuScript{K}\text{-cell}$ is the smallest set of maps that contains $\EuScript{K}$ and is closed under transfinite compositions, pushouts and coproducts. 

The smallness condition above holds in the following general situations:
\begin{enumerate}
	\item[(a)] (\textit{Combinatorial}) If the underlying category $\Mrect$ is presentable, every object is small with respect to the whole category $\Mrect$. Hence, Quillen's soa works for any set of maps $\EuScript{K}$.
	%%\item[(b)] Assume that $\Mrect$ admits a proper, well-copowered strong factorization system with right class $\mathcal{M}$. If for every object $\Xrect\in\Mrect$ there is a regular cardinal $\upkappa_{\Xrect}$ such that $\Mrect(\Xrect,\star)$ sends $\upkappa_{\Xrect}$-filtered unions of $\mathcal{M}$-subobjects to $\upkappa_{\Xrect}$-filtered unions of sets, then Garner's soa works for any small category of maps.  AQUI NO, PORQUE NECESITA GARNER SOA.
	\item[(b)] (\textit{Cellular}) Suppose that $\Mrect$ contains a set of maps $\EuScript{I}$ whose domains and codomains are compact relative to $\EuScript{I}$ (Definition \cite[Definition 10.8.1]{hirschhorn_model_2003}) and such that $\EuScript{I}\text{-cell}$ is contained in monomorphisms. Then, any $\EuScript{I}$-cofibrant object is small relative to ${}^{\boxslash}(\EuScript{I}^{\boxslash})$. See \cite[Chapter 12]{hirschhorn_model_2003} for the results that imply this claim. Hence, any set of morphisms $\EuScript{K}$ belonging to ${}^{\boxslash}(\EuScript{I}^{\boxslash})$ whose domains are $\EuScript{I}$-cofibrant admits Quillen's soa.
\end{enumerate}

The drawback for Quillen's soa is: when constructing the factorization of a map, the iterative construction does not pay attention to solutions of lifting problems that were present on previous steps. Garner in \cite{garner_understanding_2009} fixed this issue with a clever modification of the iterative construction. His modified soa enjoys better categorical properties than Quillen's and can be adapted to work in more general settings (see \cite[Chapter 12]{riehl_categorical_2014}). 

We will consider the easiest case where Garner's soa can be applied. This will be the one that we will need later to produce Bousfield localizations and to discuss the axioms for cellular model categories. For a set of maps $\EuScript{K}$, Garner's soa really produces an algebraic weak factorization system $(\mathbb{C}_{\EuScript{K}},\mathbb{F}_{\EuScript{K}})$ (\cite[Definition 2.9]{garner_understanding_2009}) whose underlying weak factorization system is $({}^{\boxslash}(\EuScript{K}^{\boxslash}),\EuScript{K}^{\boxslash})$. In particular, for a map $\upf$, Garner's soa yields a factorization
$$
\upf\colon \bullet\xrightarrow{\quad \mathbb{C}_\EuScript{K}\text{-coalg}\quad}\bullet\xrightarrow{\quad\mathbb{F}_\EuScript{K}\text{-alg}\quad}\bullet.
$$
One of the easiest improvements that Garner's soa has over Quillen's is that it can be applied under weaker smallness conditions. For instance:
\begin{enumerate}
	\item[(c)] Assume that $\Mrect$ admits a proper, well-copowered strong factorization system with right class $\mathcal{M}$. If for every object $\Xrect\in\Mrect$ there is a regular cardinal $\upkappa_{\Xrect}$ such that $\Mrect(\Xrect,\star)$ sends $\upkappa_{\Xrect}$-filtered unions of $\mathcal{M}$-subobjects to $\upkappa_{\Xrect}$-filtered unions of sets, then Garner's soa works for any set of maps.
\end{enumerate}

\begin{rem}
	Chorny \cite{chorny_generalization_2006} and Christensen-Isaksen \cite{christensen_duality_2004} have proposed small object arguments for non-cofibrantly generated situations, i.e. when one does not start from sets of maps to which apply soa.
\end{rem}

%AQUI QUIERO DECIR QUE SI LOS I-cell SON MONOS, COMPACTO IMPLICA SMALL Y POR TANTO TODO OBJETO COFIBRANTE ES SMALL CON RESPECTO A LAS COFIBRACIONES. ESTO PERMITE APLICAR EL SOA PARA CUALQUIER CONJUNTO DE COFIBRACIONES QUE EMPIECEN EN UN OBJETO SMALL CON RESPECTO A I, OBJETOS COFIBRANTES O LAS SOURCES DE J (ESENCIALMENTE).

\paragraph{Cellular complexes and their intersections.}

%\textcolor{blue}{Work in progress}

 Note that in Quillen's soa, the class of maps $\EuScript{K}\text{-cell}$ is particularly important. In fact, the study of classes of relative cell complexes is essential for several questions that one may ask for cofibrantly generated model structures (e.g. showing that a category carries a model structure or that a Quillen adjunction is an equivalence, etc).  Due to our motivation on Bousfield localizations, we observe that Hirschhorn \cite{hirschhorn_model_2003} performs a detailed analysis of $\EuScript{K}\text{-cell}$ with an eye towards this application. 
 
 Aside a cardinality control that he needed for his Bousfield-Smith cardinality argument (succintly recalled in Remark \ref{rem_RegularCardinalForBousfieldSmithArgument}), he also needs to understand cellular subcomplexes and their intersections (Remark \ref{rem_EffectiveMonoForIntersections}). This latter point is transparently explained in \cite[Section 1.5]{goerss_moduli_2005} and we are going to focus our attention on it. Hirschhorn's solution to this problem is adhoc. He impose that relative $\EuScript{K}\text{-cell}$ complexes are  effective monomorphisms and hence a simple categorical argument yields that intersections of two cellular subcomplexes exist and are given by picking common cells (paragraph around \cite[Diagram (1.5.1)]{goerss_moduli_2005}). Of course, this leaves open the question of when more general intersections of subcomplexes exist and also adds a difficult axiom to check in practice. We propose a plan to solve these issues by further studying the subcategory of maps $\mathbb{C}_{\EuScript{K}}$-coalg that plays the role of $\EuScript{K}\text{-cell}$ in Garner's soa. 

 Before stating the plan, it is important to note that the following conditions on the set $\EuScript{K}$, which are part of the definition of cellular model category, 
 \begin{itemize}
 	\item[($i$)] domains and codomains of maps in $\EuScript{K}$ are compact relative to $\EuScript{K}$,
 	\item[($ii$)] the class $\EuScript{K}\text{-cell}$ is contained in monomorphisms,
 \end{itemize}
 may be taken for granted. Those are sufficient to ensure that Quillen's or Garner's soa applies to $\EuScript{K}$. Moreover, \cite[Remark 12.5.6]{riehl_categorical_2014} tells us that ($ii$) simplifies Garner's soa, making it a less redundant modification of Quillen's. 
 
 Under these assumptions, the first step of the plan is to relate $\mathbb{C}_{\EuScript{K}}\text{-coalg}$ and $\EuScript{K}\text{-cell}$ using recent ideas from Athorne \cite{athorne_coalgebraic_2012}. The strategy is to define a category of nicely presented $\EuScript{K}$-cell complexes over the arrow category $\Mrect^{\mathbb{2}}$, generalizing the notion of relative cell complexes in \cite{athorne_coalgebraic_2012} by changing the cardinal that bounds the sequence of strata, and checking that their category is equivalent to $\mathbb{C}_{\EuScript{K}}\text{-coalg}$. Much of Athorne's work is easily generalizable, but there is an essential result, \cite[Pullback Lemma]{athorne_coalgebraic_2012}, which we do not know how to circumvent and which is not likely to hold just assuming ($i$) and ($ii$) above. 
 
 Having such identification at hand, the existence of general intersections of subcomplexes is related to completeness of $\mathbb{C}_{\EuScript{K}}\text{-coalg}$. To see why, let us explain how one intersects two subcomplexes. Let $\upi\colon\Zrect\to\Xrect\leftarrow\Yrect\colon\upj$ be a pair of subcomplexes of $\Xrect$. Their intersection, if it exists, fits into a pullback square
 $$
 \begin{tikzcd}[ampersand replacement=\&]
 \Zrect\curlywedge\Yrect\ar[r,"\upi'"]\ar[d,"\upj'"'] \ar[rd, phantom, "\lrcorner"]\& \Yrect\ar[d, "\upj"]\\
 \Zrect\ar[r,"\upi"'] \& \Xrect
 \end{tikzcd}
 $$
 in the category of $\EuScript{K}$-cell complexes and $\EuScript{K}$-cell inclusions between them. Under existence of pullbacks in $\mathbb{C}_{\EuScript{K}}\text{-coalg}$, one may construct $\Zrect\curlywedge\Yrect$ and its structural maps $\upi',\,\upj'$ by forming the following pullbacks in this category of coalgebras
 $$
 \begin{tikzcd}[ampersand replacement=\&]
 (\mathbb{0}\to\Zrect\curlywedge\Yrect)\ar[r,"(\id\text{,}\upi')"]\ar[d,"(\id\text{,}\upj')"'] \ar[rd, phantom, "\lrcorner"]\& (\mathbb{0}\to\Yrect)\ar[d, "(\id\text{,}\upj)"]\\
 (\mathbb{0}\to\Zrect)\ar[r,"(\id\text{,}\upi)"'] \& (\mathbb{0}\to\Xrect)
 \end{tikzcd} \quad \text{and} \quad
 \begin{tikzcd}[ampersand replacement=\&]
 (\Zrect\curlywedge\Yrect\xrightarrow{\upj'}\Zrect)\ar[r,"(\upi'\text{,}\upi)"]\ar[d,"(\upj'\text{,}\id)"'] \ar[rd, phantom, "\lrcorner"]\& (\Yrect\to\Xrect)\ar[d, "(\upj\text{,}\id)"]\\
 (\Zrect\to\Zrect)\ar[r,"(\upi\text{,}\upi)"'] \& (\Xrect\to\Xrect)
 \end{tikzcd}.
 $$
 The first one proves that $\Zrect\curlywedge\Yrect$ is a $\EuScript{K}$-cell complex and the second one that $\upj'$ is a $\EuScript{K}$-cellular map (an analogous pullback shows that $\upi'$ is also $\EuScript{K}$-cellular).
 
 What is gained by using a coalgebraic description is that $\mathbb{C}_{\EuScript{K}}\text{-coalg}$ is complete by condition ($ii$) if we assume that $\Mrect$ is well-powered \cite[Proposition 2.10]{hess_homotopy_2014}.  

\begin{rem} This program is not concluded mainly due to the lack of a replacement for \cite[Pullback Lemma]{athorne_coalgebraic_2012}. Also, to be able to apply intersections $\Zrect\curlywedge\Yrect$ as constructed above as a replacement of Hirschhorn's intersections of subcomplexes, which we denote in this work by $\Zrect\cap\Yrect$, to construct Bousfield localizations, an exhaustive analysis of $\Zrect\curlywedge\Yrect$ is yet required. Despite all this, filling these holes would allow one to change the hardest axiom of cellular model structures ($\EuScript{K}\text{-cell}$ consists of effective monomorphisms) by more natural conditions on the underlying category (such as $\Mrect$ is well-powered).
\end{rem}



%
%
%
%
%
%
%
%
%
%Of course, a coalgebraic presentation of cellular cofibrations yields automatically all colimits that you may form, but under additional hypothesis it also brings at our disposal limits. That is how we form intersections of cellular complexes, answering a question of Hopkins.    
%
%
%
%
%
%
%
%
%Athorne identification to enhance $\Irect\text{-cell}$ to  $\Irect\text{-CellCplx}$ and so construct colimits (automatic) and limits of subcells. Reference Goerss-Hopkins.




